A general approach to posterior contraction in nonparametric inverse problems

In this paper we propose a general method to derive an upper bound for the contraction rate of the posterior distribution for nonparametric inverse problems. We present a general theorem that allows us to derive con- traction rates for the parameter of interest from contraction rates of the related direct problem of estimating transformed parameter of interest. An interesting aspect of this approach is that it allows us to derive con- traction rates for priors that are not related to the singular value decomposition of the operator. We apply our result to several examples of linear inverse problems, both in the white noise sequence model and the nonparametric regression model, using priors based on the singular value decomposition of the operator, location-mixture priors and splines prior, and recover minimax adaptive contraction rates.

==> Parts/old/extremely_old.tex <==
In this section we consider the white noise setting with truncated
Gaussian priors. The main purpose of this part is to show that, in
contrast to what was obtained before, in some classes of ill-posed problems
adaptation does not need to be achieved simultaneously in both direct and indirect problem.
As a matter of fact, in this part the rates in the direct problem will be much (polynomially)
slower than the optimal rates. This is mostly due to the fact that we consider in here
severely and extremely ill-posed problems that yield logarithmic rates of recovery. 
See also \cite{KVZ13} and \cite{Agapiou14} for examples.

We consider the white noise setting, where we observe
%
\[
%
    Y_i = \kappa_if_i + \frac{1}{\sqrt{n}}Z_i,
%
\]
%
where $\kappa_i \asymp \exp(-\gamma i^p)$ for some $p \geq 1$ and $\gamma > 0$, and
$Z_1, Z_2, \ldots$ are independent standard normal random variables. Let
$Kf$ denote the sequence $\kappa_if_i$. The $\ell_2$-norm is denoted by $\|\cdot\|$.


We first consider estimation of $Kf_0$ that will be later used to obtain the rate
of contraction of the posterior around $f_0$. We put a product prior on $f$ of
the form
%
\[
%
\Pi = \bigotimes_{i=1}^{k_n} N(0, \lambda_i),
%
\]
%
where $\lambda_i = i^{-\alpha}\exp(-\xi i^p)$, for $\alpha \geq 0$, 
and some $k_n \to \infty$. 

There are two choices of $k_n$ leading to the optimal rate of recovery, 
both motivated by a specific step in the proof of the main theorem of 
this section: the square bias comprises of two terms depending on $k_n$ 
that should be of the same order.

Firstly, we can choose 
$k_n$ solving $1 = n\lambda_i\exp(-2\gamma i^p) = ni^{-\alpha}\exp(-(\xi+2\gamma)i^p)$. 
Using the Lambert function $W$ one can show that
%
\begin{equation}
\label{eq:k_n}
%
    k_n = \Bigl(\frac{\alpha}{p(\xi+2\gamma)}
            W\Bigl(n^{\frac{p}{\alpha}}\frac{p(\xi+2\gamma)}{\alpha}\Bigr)\Bigr)^{1/p}
        = \Bigl(\frac{\log n}{\xi+2\gamma} + O(\log\log n)\Bigr)^{1/p},
%
\end{equation}
%
see also Lemma A.4. in \cite{KVZ13}. Note that in this case we have 
$\exp(k_n^p) = (nk_n^{-\alpha})^{1/(\xi+2\gamma)}$. Therefore,  we do not have to 
specify the constant in front of the $\log\log n$ term 
in the definition of $k_n$.

The two terms constituting the square bias can be also balanced 
in order to achieve an optimal upper bound. This leads to 
the following choice of $k_n$
%
\begin{equation}
\label{eq:k_n_bis}
%
    \tilde k_n = \Bigl(\frac{\log n}{\xi+2\gamma} - \frac{\alpha}{p}\cdot\frac{\log\log n}{\xi+2\gamma}\Bigr)^{1/p}.
%
\end{equation}

It can be shown that $k_n^p-\tilde k_n^p = o(\log\log n)$. Note that the parameters 
of the prior do not depend on $f_0$, but only on $K$, which is known. For 
the sets $\mathcal{S}_n$ we choose the sets defined as in (\ref{eq:Sn}) 
with $k_n$ as above and $c = 0$. Therefore, the prior is supported on $\mathcal{S}_n$ 
and the first condition of Theorem~\ref{thm:main} is trivially satisfied.

\begin{theorem}
Suppose the true $f_0$ belongs to $S^\beta$ for $\beta > 0$. 
Then for every $R > 0$ and $M_n \to \infty$
%
\[
%
    \sup_{\|f_0\|_\beta \leq R}
	  \E_0\Pi_n\bigl(f: \|f-f_0\| \geq M_n(\log n)^{-\beta/p}\bigm|Y\bigr)\to 0.
%
\]
%
\end{theorem}

\begin{proof}
Assume for brevity that we have the exact equality $\kappa_i = \exp(-\gamma i^p)$.
Dealing with the general case is straightforward, but makes the proofs somewhat
lengthier.

Since $Y_i | f_i \sim N(\kappa_if_i, n^{-1})$ and $f_i \sim N(0, \lambda_i)$
for $i \leq k_n$,
we have the following posterior distribution (for $Kf$):
%
\[
%
    Kf | Y \sim \bigotimes_{i=1}^{k_n}
      N\Bigl(\frac{n\lambda_i\kappa_i^2}{1+n\lambda_i\kappa_i^2}Y_i,
             \frac{\lambda_i\kappa_i^2}{1+n\lambda_i\kappa_i^2}\Bigr).
%
\]
%
The posterior is denoted by $\Pi_n(\, \cdot \, | Y)$ and we also let
%
\[
%
    s_{i,n} = \frac{\lambda_i\kappa_i^2}{1+n\lambda_i\kappa_i^2},
    \qquad
    t_{i,n} = \frac{n\lambda_i^2\kappa_i^4}{(1+n\lambda_i\kappa_i^2)^2}.
%
\]
%
Since the posterior is Gaussian, we have
%
\begin{equation}\label{eq:postrisk}
%
    \int\|Kf-Kf_0\|^2\, d\Pi_n(Kf|Y) = \|\widehat{Kf}-Kf_0\|^2+\sum_{i=1}^{k_n}s_{i,n},
%
\end{equation}
%
where $\widehat{Kf}$ denotes the posterior mean and can be rewritten as:
%
\[
\begin{split}
%
    \widehat{Kf} &= \Bigl(\frac{n\lambda_i\kappa_i^2}{1+n\lambda_i\kappa_i^2}Y_i\Bigr)_{i=1}^{k_n}
    = \Bigl(\frac{n\lambda_i\kappa_i^3f_{0,i}}{1+n\lambda_i\kappa_i^2}
      + \frac{\sqrt{n}\lambda_i\kappa_i^2Z_i}{1+n\lambda_i\kappa_i^2}\Bigr)_{i=1}^{k_n}\\
    &=: \E\widehat{Kf} + (\sqrt{t_{i,n}}Z_i)_{i=1}^{k_n}.
%
\end{split}
\]


By Markov's inequality the left side of (\ref{eq:postrisk}) is an upper bound to
$M_n^2\epsi_n^2$ times the desired posterior probability. Therefore, in order to show that
$\Pi_n(f: \|Kf-Kf_0\| \geq M_n\epsi_n|Y)$ goes to zero in probability, it suffices to show
that the expectation (under the true $f_0$) of the right hand side of (\ref{eq:postrisk}) is
bounded by a multiple of $\epsi_n^2$. The last term is deterministic. As for the first
term we have
%
\[
%
    \E\|\widehat{Kf}-Kf_0\|^2 = \|\E\widehat{Kf}-Kf_0\|^2 + \sum_{i=1}^{k_n} t_{i,n}.
%
\]
%
We also observe
%
\[
%
    \|\E\widehat{Kf}-Kf_0 \|^2 
	   = \sum_{i=1}^{k_n} \frac{\kappa_i^2f_{0,i}^2}{(1+n\lambda_i\kappa_i^2)^2} 
	      + \sum_{i=k_n+1}^\infty \kappa_i^2 f_0^2.
%
\]

We are interested in the asymptotics of the three sums
%
\begin{equation*}\label{eq:threesums}
%
    \sum_{i=1}^{k_n} \frac{\kappa_i^2f_{0,i}^2}{(1+n\lambda_i\kappa_i^2)^2}
		+ \sum_{i=k_n+1}^\infty \kappa_i^2 f_{0,i}^2, \quad
    \sum_{i=1}^{k_n} s_{i,n}, \quad
    \sum_{i=1}^{k_n} t_{i,n}.
%
\end{equation*}
%
To deal with all these sums we use lemmas in \cite{KVZ13}, after straightforward modifications.
(We note that $k_n \asymp I_n$, and we only deal with the first part of the sum in the latter two cases).
We obtain (using either (\ref{eq:k_n}) or (\ref{eq:k_n_bis}))
%
\begin{equation}
\label{eq:asymptotics}
\begin{split}
%
    \sum_{i=1}^{k_n} \frac{\kappa_i^2f_{0,i}^2}{(1+n\lambda_i\kappa_i^2)^2}
        + \sum_{i=k_n+1}^\infty \kappa_i^2 f_{0,i}^2
    &\lesssim \|f_0\|^2_\beta n^{-\frac{2\gamma}{\xi+2\gamma}}(\log n)^{-\frac{2\beta}{p}+\frac{2\gamma\alpha}{p(\xi+2\gamma)}},\\
    \sum_{i=1}^{k_n} s_{i,n} \asymp \sum_{i=1}^{k_n} t_{i,n} &\asymp n^{-1}(\log n)^{\frac{1}{p}}.
%
\end{split}
\end{equation}
%
This shows that both the posterior spread and the variance of the posterior mean are
in this case of the correct order $n^{-1}(\log n)^{1/p}$ (i.e., when we consider estimation
of the analytically smooth truth $Kf_0$). However, the bias term is too slow. This is
presumably not surprising since the prior on $f$ was analytic, whereas the truth was Sobolev.

Summing up, the posterior contraction rate for the direct problem is given by
%
\[
%
    \epsi_n = (\log n)^{-\frac{\beta}{p}+\frac{\gamma\alpha}{p(\xi+2\gamma)}} n^{-\frac{\gamma}{\xi+2\gamma}}
%
\]

By (\ref{eq:mod}) an upper bound for the modulus of continuity is given by 
(with either (\ref{eq:k_n}) or (\ref{eq:k_n_bis})) 
%
\begin{align*}
%
	\omega(\mathcal{S}_n,f_0, \|\cdot\|, \|\cdot\|,M_n\epsilon_n) 
	&\lesssim M_n \exp(\gamma k_n^p) \epsilon_n + k_n^{-\beta}\\
	&\lesssim M_n n^{\frac{\gamma}{\xi+2\gamma}} (\log n)^{-\frac{\gamma\alpha}{p(\xi+2\gamma)}} \epsilon_n + (\log n)^{-\frac{\beta}{p}}\\
	&\lesssim M_n (\log n)^{-\frac{\beta}{p}},
,
%
\end{align*}
%
which ends the proof.
\end{proof}

\begin{lemm}The inequalities in (\ref{eq:asymptotics}) hold. (Does not need to be included in the final manuscript, although some parts of 
the proof might be transferred to the main proof.)
\end{lemm}

\begin{proof}
We first note that 
%
\[
%
	\bigl(\log n + O(\log\log n)\bigr)^{1/p} 
	= (\log n)^{1/p}\bigl(1+o(\log n)\bigr)^{1/p}\footnote{\bartek{Can we drop the latter $1/p$?}},
%
\]
%
so if $k_n$ is exponentiated, we might assume it is of the order $(\log n)^{1/p}$. Note 
that for $k_n$ as in (\ref{eq:k_n}) we have $\exp(k_n^p) = (nk_n^{-\alpha})^{1/(\xi+2\gamma)}$ 
and we can express the upper bounds in terms of powers of $k_n$, i.e., without $\exp(k_n^p)$. 
The same holds for exponentiated $k_n$ as in (\ref{eq:k_n_bis}). However, in this case expressions 
with $\exp(k_n^p)$ cannot be simplified and we then need to use $k_n$ exactly as in (\ref{eq:k_n_bis}).

Note that $t_{i,n} \leq n^{-1}$ and $s_{i,n} \leq n^{-1}$. 
Therefore, the last two sums in (\ref{eq:asymptotics}) are bounded from 
above by $n^{-1}k_n = n^{-1}(\log n)^{1/p}$.

Regardless of the choice of $k_n$, for the first term in the first sum in (\ref{eq:asymptotics}) we have
%
\[
\begin{split}
%
	\sum_{i=1}^{k_n} \frac{\kappa_i^2f_{0,i}^2}{(1+n\lambda_i\kappa_i^2)^2} &\leq 
	n^{-2} \sum_{i=1}^{k_n} \lambda_i^{-2}\kappa_i^{-2}i^{-2\beta}i^{2\beta}f_{0,i}^2\\
	&= n^{-2} \sum_{i=1}^{k_n} i^{2(\alpha-\beta)}\exp(2(\xi+\gamma)i^p)i^{2\beta}f_{0,i}^2,
%
\end{split}
\]
%
and for $k_n$ large enough all terms $i^{2(\alpha-\beta)}\exp(2(\xi+\gamma)i^p)$ are dominated 
by $k_n^{2(\alpha-\beta)}\exp(2(\xi+\gamma)k_n^p)$, so
%
\begin{equation}
\label{eq:firstsum}
%
	\sum_{i=1}^{k_n} \frac{\kappa_i^2f_{0,i}^2}{(1+n\lambda_i\kappa_i^2)^2} \leq
	 n^{-2}k_n^{2(\alpha-\beta)}\exp(2(\xi+\gamma)k_n^p)\|f_0\|^2_\beta.
%
\end{equation}

As for the second term in the first sum in (\ref{eq:asymptotics}) we note that
%
\[
%
	\sum_{i=k_n+1}^\infty \kappa_i^2 f_{0,i}^2 = \sum_{i=k_n+1}^\infty \exp(-2\gamma i^p)i^{-2\beta}i^{2\beta} f_{0,i}^2,
%
\]
%
and since $\exp(-2\gamma i^p)i^{-2\beta}$ is monotone decreasing
%
\begin{equation}
\label{eq:secondsum}
%
	\sum_{i=k_n+1}^\infty \kappa_i^2 f_{0,i}^2 
	  \leq \exp(-2\gamma k_n^p)k_n^{-2\beta}\|f_0\|^2_\beta.
%
\end{equation}

If $k_n$ is as in (\ref{eq:k_n}), recall that $\exp(k_n^p) = (nk_n^{-\alpha})^{1/(\xi+2\gamma)}$  
and therefore we can rewrite the bounds in (\ref{eq:firstsum}) and (\ref{eq:secondsum}) 
as
%
\[
%
	n^{-2}k_n^{2(\alpha-\beta)}\bigl(nk_n^{-\alpha}\bigr)^{\frac{2(\xi+\gamma)}{\xi+2\gamma}} =  
	n^{-\frac{2\gamma}{\xi+2\gamma}} k_n^{-2\beta + \frac{2\gamma\alpha}{\xi+2\gamma}},
%
\]
%
and
%
\[
%
	k_n^{-2\beta}\bigl(nk_n^{-\alpha}\bigr)^{-\frac{2\gamma}{\xi+2\gamma}} = 
	n^{-\frac{2\gamma}{\xi+2\gamma}} k_n^{-2\beta + \frac{2\gamma\alpha}{\xi+2\gamma}}.
%
\]
%
Finally, since $k_n$ in this case can be taken of the order $(\log n)^{1/p}$, we obtain the 
desired upper bound.

If we want to obtain $k_n$ as in (\ref{eq:k_n_bis}), we first need to assume that
%
\[
%
	k_n = \bigl(C_1\log n + C_2 \log\log n\bigr)^{1/p},
%
\]
%
and then substitute such $k_n$ in (\ref{eq:firstsum}) and (\ref{eq:secondsum}). Note that 
again if $k_n$ is only exponentiated, we can substitute $k_n = (\log n)^{1/p}$. 
This procedure will lead to us to $k_n$ as in (\ref{eq:k_n_bis}), and also the 
desired upper bound.
\end{proof}




==> Parts/old/mildly_scaling_incomplete.tex <==
%!TEX root = ../Inv_notes2.tex

Our first example is based on the well-studied infinite-dimensional 
normal mean model. In the Bayesian context the problem of direct 
estimation of infinitely many means has been studied, among others, by 
\cite{Zhao, Belitser, GhosalVdv07, Shen2001}. 
\bartek{MORE!}

We consider the white noise setting, where we observe an infinite 
sequence $Y^n=(Y_1, Y_2, \ldots)$ satisfying 
%
\[
%
    Y_i = \kappa_if_i + \frac{1}{\sqrt{n}}Z_i,
%
\]
%
where $\kappa_i \asymp i^{-p}$ for some $p \geq 0$, and
$Z_1, Z_2, \ldots$ are independent standard normal random variables. Let
$Kf$ denote the sequence $\kappa_if_i$, and the $\ell_2$-norm is denoted
by $\|\cdot\|$. In this setting $\H_1=\H_2=\ell_2$. 

We put a product prior on $f$ of the form
%
\[
%
\Pi = \bigotimes_{i=1}^{\infty} N(0, \lambda_i),
%
\]
%
where $\lambda_i = i^{-1-2\alpha}$, for some $\alpha > 0$.
Furthermore, the true parameter $f_0$ belongs to $S^\beta$ for some
$\beta > 0$, that is, it satisfies
%
\[
%
    \|f_0\|_\beta^2 = \sum f_{0,i}^2i^{2\beta} < \infty.
%
\]
%
Therefore, $\|Kf_0\|_{\beta+p}^2$ is finite, and one can deduce from 
the results of \cite{Belitser, Zhao} that 
\[
%
    \E_0\Pi_n\bigl(f: \|Kf-Kf_0\| \geq M_n\epsilon_n\bigm|Y^n\bigr)\to 0,
%
\]
%
where
%
\[
%
    \epsilon_n = (n\tau_n^2)^{-\frac{\beta+p}{1+2\alpha+2p}\wedge 1}
        + \tau_n(n\tau_n^2)^{-\frac{\alpha+p}{1+2\alpha+2p}}
%
\]


Let $k_n = C_2(n\tau_n^2)^{1/(1+2\alpha+2p)}$ for an arbitrary $C_2 > 0$, 
and $c = 8(1+2\alpha)/\alpha$ in (\ref{eq:Sn}), thus
%
\[
%
    \omega(\mathcal{S}_n,\un{\cdot}, \deux{\cdot},\delta)
    \asymp (n\tau_n^2)^{-\frac{p}{1+2\alpha+2p}}\delta.
%
\]
%
For $W_1, W_2, \ldots$ independent standard normal random variables
%
\[
\begin{split}
%
    \Pi(\mathcal{S}_n) &= \Pr\Bigl(\sum_{i>k_n} \lambda_iW_i^2
            \leq c\sum_{i \leq k_n}\lambda_iW_i^2\Bigr) \\
        &\geq \Pr\Bigl(\sum_{i>k_n} \lambda_iW_i^2
            \leq \frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}\Bigr)
            \Pr\Bigl(\frac{\tau_n^2k_n^{-2\alpha}}{8}
            \leq \sum_{i \leq k_n}\lambda_iW_i^2\Bigr).
%
\end{split}
\]
%

Let us first deal with the first term. For some $t > 0$
%
\begin{align*}
%
    \Pr\Bigl(\sum_{i>k_n} \lambda_iW_i^2
            &> \frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}\Bigr)\\
        &= \Pr\Bigl(\exp\Bigl(t\sum_{i>k_n} \lambda_iW_i^2\Bigr)
            > \exp\Bigl(t\frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}\Bigr)\Bigr)\\
        &\leq \exp\Bigl(-t\frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}\Bigr)
            \E \exp\Bigl(t\sum_{i>k_n} \lambda_iW_i^2\Bigr)\\
%        &= \exp\Bigl(-t\frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}\Bigr)
%            \E\prod_{i>k_n} \exp(t\lambda_iW_i^2)\\
        &= \exp\Bigl(-t\frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}\Bigr)
            \prod_{i>k_n} \E\exp(t\lambda_iW_i^2)\\
        &= \exp\Bigl(-t\frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}\Bigr)
            \prod_{i>k_n} (1-2t\lambda_i)^{-1/2}.
%
\end{align*}
%
We first applied Markov's inequality, and later used properties of
the moment generating function. Here we additionally assume
that $2t\lambda_i < 1$ for $i > k_n$.

We continue with the logarithm of the right-hand side of the
previous display. Since $\log(1-y)\geq -y/(1-y)$, we have
%

{ \color{red}
    There is indeed a problem here, because the choice of $t$ bellow leads to bound $-t\frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}
            + \sum_{i>k_n}\log (1-2t\lambda_i)^{-1/2}$ by $0$... here are some quick computations (that may need to be double checked) that should fix things.
    We want to control the 2nd term (sum of logs), so we have using a series-integral comparison

\begin{align*}
-\frac{1}{2} \sum_{i>k_n} \log(1 - 2t\tau_n^2 i^{-1-2\alpha}) &\leq -\frac{1}{2} \int_{k_n}^{\infty} \log(1-2t\tau_n^2x^{-1-2\alpha}) dx ~ \text{integr. by parts...} \\ 
& = -\frac{1}{2} \left( -k_n \log(1-2t\tau_n^2 k_n^{-1-2\alpha}) - (2\alpha +1) 2t\tau_n^2 \int_{k_n}^\infty  {x^{-1-2\alpha} \over 1-2t\tau_n^2x^{-1-2\alpha}  } dx \right) \\
& \leq -\frac{1}{2} \left( -k_n \log(1-2t\tau_n^2 k_n^{-1-2\alpha}) - (2\alpha +1) {2t\tau_n^2 \over 1-2t\tau_n^2 k_n^{-1-2\alpha}  } \int_{k_n}^\infty  {x^{-1-2\alpha}  } dx \right) \\ 
&\leq -\frac{1}{2} \left( -k_n \log(1-2t\tau_n^2 k_n^{-1-2\alpha}) - (2\alpha +1) {2t\tau_n^2 \over 1-2t\tau_n^2 k_n^{-1-2\alpha}  } {k_n^{-2\alpha} \over 2\alpha } \right)
\end{align*}
Now taking $t = c \tau_n^{-2} k_n^{-2\alpha - 1}$ we have for a well chosen $c \leq 1/4$ 

\begin{multline*}
-t\frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}-\frac{1}{2} \sum_{i>k_n} \log(1 - 2t\tau_n^2 i^{-1-2\alpha})  \\ \leq \frac{k_n}{2} \log(1-2c) + \frac{1+2\alpha}{2\alpha} \frac{c k_n}{1-2c} - ck_n \frac{1+2\alpha}{\alpha} \\ \leq - C_\alpha k_n  
\end{multline*}

where $0<C_\alpha$ is some constant that only depends on $c$ and $\alpha$
}
\begin{align*}
%
    -t\frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}
            + &\sum_{i>k_n}\log (1-2t\lambda_i)^{-1/2}\\
        &=  -t\frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}
            - \frac{1}{2} \sum_{i>k_n}\log (1-2t\lambda_i)\\
        &\leq -t\frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}
            + \frac{1}{2} \sum_{i>k_n}\frac{2t\lambda_i}{1-2t\lambda_i}\\
        &\leq -t\frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}
            + \frac{2t\tau_n^2}{1-2t\tau_n^2k_n^{-1-2\alpha}}
                \sum_{i>k_n}i^{-1-2\alpha}\\
        &\leq -t\frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}
            + \frac{1+2\alpha}{\alpha}
                \frac{2t\tau_n^2}{1-2t\tau_n^2k_n^{-1-2\alpha}} k_n^{-2\alpha}.
%
\end{align*}
%
Thus for $t = \tau_n^{-2}k_n^{1+2\alpha}/4$
%
\[
%
    \Pr\Bigl(\sum_{i>k_n} \lambda_iW_i^2 > \frac{1+2\alpha}{\alpha}\tau_n^2k_n^{-2\alpha}\Bigr)
    \leq \exp\Bigl(-\frac{1+2\alpha}{8\alpha}k_n\Bigr).
%
\]
%
We proceed with the second term along the same lines and arrive at
%
\[
%
    \Pr\Bigl(\sum_{i\leq k_n} \lambda_iW_i^2 < \frac{\tau_n^2k_n^{-2\alpha}}{8}\Bigr) \leq \exp\Bigl(-\frac{k_n}{8}\Bigr).
%
\]
%

Combining both bounds we obtain
%
\begin{align*}
%
    \Pi(\mathcal{S}_n) &\geq \Bigl(1-\exp\Bigl(-\frac{1}{8}k_n\Bigr)\Bigr)
            \Bigl(1-\exp\Bigl(-\frac{1+2\alpha}{8\alpha}k_n\Bigr)\Bigr)\\
        &\geq \Bigl(1-\exp\Bigl(-\frac{1}{8}k_n\Bigr)\Bigr)^2 \geq 1-\exp\Bigl(-\frac{1}{16}k_n\Bigr),
%
\end{align*}
%
where the last inequality holds for $n$ large enough.
%
%\subsubsection*{Head}
%
%We now consider the beginning of the sum. Similarly as before we obtain for
%$t > 0$
%%
%\begin{align*}
%%
%    \Pr\Bigl(\sum_{i\leq k_n} \lambda_iW_i^2 < b\Bigr) &=  \Pr\Bigl(\exp\Bigl(-t\sum_{i\leq k_n} \lambda_iW_i^2\Bigr) > \exp(-tb)\Bigr)
%           \leq \exp(tb)\E \exp\Bigl(-t\sum_{i\leq k_n} \lambda_iW_i^2\Bigr)\\
%      &= \exp(tb) \E\prod_{i\leq k_n} \exp(-t\lambda_iW_i^2)
%          = \exp(tb) \prod_{i\leq k_n} \E\exp(-t\lambda_iW_i^2)\\
%      &= \exp(tb) \prod_{i\leq k_n} (1+2t\lambda_i)^{-1/2}.
%%
%\end{align*}
%%
%We again used Markov's inequality and properties of the moment generating function. Note
%there is no additional assumption on $t$.
%
%We continue with the logarithm of the right-hand side of the previous display. Since $\log(1+y)\geq y/(1+y)$, we have
%%
%\begin{align*}
%%
%    tb + \sum_{i\leq k_n}\log (1+2t\lambda_i)^{-1/2} &=  tb - \frac{1}{2} \sum_{i\leq k_n}\log (1+2t\lambda_i)
%      \leq tb - \frac{1}{2} \sum_{i\leq k_n}\frac{2t\lambda_i}{1+2t\lambda_i}.
%\end{align*}
%%
%Assuming that $t> k_n^{1+2\alpha}/2$, we have  $1+2t\lambda_i<4t\lambda_i$ for $i \leq k_n$, thus
%%
%\begin{align*}
%%
%    tb - \frac{1}{2} \sum_{i\leq k_n}\frac{2t\lambda_i}{1+2t\lambda_i}
%       &\leq tb - \frac{1}{4}k_n.
%%
%\end{align*}
%%
%Taking $t = k_n^{1+2\alpha}$ and $b = k_n^{-2\alpha}/8$ we arrive at
%

Moreover, since in the white noise model the $\ell_2$ balls and Kullback--Leibler
neighborhoods are equivalent, Lemma~6.3 in \cite{Belitser} suggest that (still to be checked and perhaps reformulated)
%
\[
%
    \Pi(B_n(Kf_0, \epsilon_n)) \gtrsim \exp(-n\epsilon_n^2).
%
\]
%




==> Parts/old/regression_old.tex <==
\subsubsection{SVD and orthonormal decompositions}

\subsubsection{Inverse regression using splines for the Voltera operator}
In this section, we consider the following inverse regression 
\begin{equation}
y_i = Kf(x_i) + \sigma \epsilon_i
\label{eq:model:spline:voltera}
\end{equation}
where $\epsilon \overset{iid}{\sim} \mathcal{N}(0,1)$ and $x_i$ are fixed in $[0,1]$. Here, we consider $K$ to be the Voltera operator that is $Kf$ is such that the derivative $(Kf)'=f$. We build a prior on $f$ through $K$ by considering 
$$
Kf(x) = \sum_{j=1}^J a_j B_{j,q}(x) 
$$
where $(B_{j,q})_j$ is the B-spline basis of order $q$ associated with $J$ equally spaced knots. Given the definition of $B_{j,q}$ in \citet{de1978practical}, standard computation gives 
$$
B_{j,q}'(x) = \frac{1}{J} \left( B_{j,q-1}(x) - B_{j+1,q-1}(x) \right)
$$
which in turns give
$$
f(x) = \frac{1}{J} \sum_{j=1}^{J-1} (a_{j+1} - a_j) B_{j,q-1}(x). 
$$ 
To compute the modulus of continuity for this model, we need to impose some conditions on the design. For $(B_{j,q})_j$ the spline basis of order $q$ let $\Sigma_n^q$ be 
$$
(\Sigma_n^q)_{i,j} = \frac{1}{n} \sum_{i=1}^n B_{i,q}(x_i) B_{j,q}(x_i).
$$
Similarly to \citet{GhosalVdv07} we ask that the design points are such that for all $\beta_1 \in \R^J$
$$
J^{-1} ||\beta_1||^2_{J} \asymp \beta_1' \Sigma_n^q \beta_1
$$
and for $\beta_2 \in \R^{J-1}$ 
$$
(J-1)^{-1} ||\beta_2||^2_{J-1} \asymp \beta_2' \Sigma_n^{(q-1)} \beta_2
$$
Given these conditions we get denoting $\Delta(a) = (a_{j+1} - a_j)_j \in \R^{J-1}$
\begin{align*}
	||f||_n^2 &= \frac{1}{J^2} \Delta(a)' \Sigma_{n}^{q-1} \Delta(a) \\
	&\lesssim \frac{1}{J^2} \frac{1}{J-1} ||\Delta(a)||_{J-1}^2 \\ 
	&\lesssim \frac{1}{J^2} \frac{1}{J-1} ||a||_J^2 \\
	&\lesssim \frac{1}{J^2} ||Kf||_n^2
\end{align*}
Denoting $\mathcal{S}_J = \{ f = \sum_{j=1}^{J-1} b_j B_{j,q-1}, b_j \in \R \}$ we get $\omega(\epsilon, ||\cdot||_n, ||\cdot||_n,\mathcal{S}_J) \leq J \epsilon$.

To apply Theorem \ref{th:main}, we first need to derive a concentrations rate for the estimation of $Kf$. Note that in this case we simply have a standard non parametric regression model with a spline prior. This model have been extensively studied in the literature as in \citet{GhosalVdv07} or \citet{JongeZantenSplines} and we can easily adapt their results to derive minimax adaptive separation rates. More precisely we have 
\begin{equation}
	y_i = Kf(x_i) + \sigma \epsilon_i 
	\label{eq:reg:splines}
\end{equation}
where $x_i$ are fixed in $[0,1]$ and $\epsilon_i \sim \mathcal{N}(0,1)$ and $\sigma >0$ is a known constant and for some $J>0$ $Kf(x) = \sum_{j=1}^J a_j B_{j,q}(x)$. We define a prior $\pi$ on $f$ by 
$$
\pi(f) = \sum_J \pi_J(J) \pi_{a,J}(a_1, \dots, a_J) 
$$
\begin{theorem}
	Let $\pi_J$ be such that there exists some constants $0 < c_d, c_u < \infty$ such that 
	$$
	e^{-c_d J L(J)} \lesssim \pi(J) \lesssim e^{-c_u J L(J)} 
	$$
	and for all $J >0$ let $\pi_{a,J}$ be such that $d\pi(a,J)/d\lambda$ is continuous and positive for all $(a_1,\dots,a_J) \in \R^J$. Thus if the true underlying regression function $Kf_0$ is $(\alpha+1)$-H\"olderian with $(\alpha +1)\leq q$ then 
	$$
	E_0^n(\pi(||Kf-Kf_0||_n \geq M (n/\log(n))^{-(\alpha+1)/(2\alpha +3)} | Y_n)) \to 0
	$$
	\label{th:adapt:cvrate:splines}
\end{theorem}
{\color{red} This is a draft version of this theorem, we certainly lose a $\log(n)$ somewhere in the rate\ldots I'll write the proof and make some corrections} 
\begin{proof} 
The proof will be postponed to Appendix afterward\ldots

We verify the conditions of Theorem $4$ of \citet{GhosalVdv07}. Following their notation denote $Kf_a = \sum_{j=1}^J a_j B_j$ and $Kf_{a_n}$ the $L_2(P_0^n)$ projection of $Kf_0$ into the $J$-dimensional set of B-splines. Let 
$$
S_n = \left\{ J \lesssim n^{1/(2\alpha+3)} a \in \R^J \right\}.
$$
We first get an upper bound for the entropy 
$$
N(\epsilon/18,\left\{ J,a \in S_n, ||Kf_0-Kf_{a}||_n \leq \epsilon \right\} d_n )
$$
Note that given the conditions on the design points $(x_i)$, we have 
\begin{multline*}
\left\{ J \leq (n/\log(n))^{1/(2\alpha+3)}, ||Kf - Kf_0||_n \leq \epsilon \right\} \subset \\ 
\left\{ J \leq (n/\log(n))^{1/2\alpha +3}, ||a - a_n||_J \lesssim \sqrt{J}\epsilon_n \right\}
\end{multline*}
For all $J$ and $C,C'>0$ some fixed constants, the $\epsilon$-covering number of the set $\left\{a \in \R^J, ||Kf - Kf_a||\leq \epsilon \right\}$ is bounded from above by the $C\sqrt{J}\epsilon$-covering number of the set $\left\{ a \in \R^J, ||a - a_n||_J \leq C'\sqrt{J}\epsilon \right\}$ which is known to be of the order $D^J$. We thus have that, denoting $J_n = (n/\log(n))^{1/2\alpha +3}$
$$
N(\epsilon/18,\left\{ J,a \in S_n, ||Kf_0-Kf_{a}||_n \leq \epsilon \right\} d_n ) \leq J_n D^{J_n}
$$
Following \citet{GhosalVdv07} we denote 
\begin{align*}
K_i &= \int \log(dP_{Kf(x_i)}/dP_{Kf_0(x_i)}) dP_{Kf(x_i)} \\
V_i &= \int\left( \log(dP_{Kf(x_i)}/dP_{Kf_0(x_i)}) - K_i \right)^2 dP_{Kf(x_i)}
\end{align*}
and 
$$
B_n(\epsilon,Kf_0) = \left\{ n^{-1} \sum_{i=1}^n K_i \leq \epsilon^2,n^{-1} \sum_{i=1}^n V_i \leq \epsilon^2 \right\}
$$
Standard computations (see the details in \citet{Salomond13}) gives that for some positive constants $C_1$ 
\begin{multline*}
B_n(\epsilon,Kf_0) \supset \left\{(a,J),  ||Kf - Kf_0||_n \leq C_1 \epsilon \right\} \supset \\  \left\{ J= J_n, a\in \R^J ||Kf - Kf_0||_n \leq C_1 \epsilon \right\} 
\end{multline*}
Given that $Kf_0$ is $(\alpha +1)$-H\"olderian, we have $||Kf_n - Kf_0||_n \lesssim J_n^{-\alpha -1}$ and $||Kf - Kf_n||_n^2 \lesssim J_n^{-1} ||a - a_n||_{J_n}^2||$. We thus deduce that 
$$ 
\pi\left( B_n(\epsilon_n,Kf_0 \right) \geq (C \epsilon_n)^{J_n} \pi(J = J_n) \gtrsim e^{-C n\epsilon_n^2} 
$$
Given the conditions on the prior on $J$ we get that $\Pi(S_n^c) \gtrsim e^{-n\epsilon_n^2}$. The conditions of Theorem 4 of \citet{GhosalVdv07} are thus satisfied. 
	
\end{proof}

\subsubsection{Mixture prior}
We now consider a mixture decomposition for $f$ in model \eqref{eq:model}. Mixture priors are common in the Bayesian literature and have been well studied in the non parametric setting {\color{red} citations needed}. In the regression setting it is common (e.g. \citet{ dejongvzanten12}) to consider mixtures of kernels. Let $\Phi_i$ be a kernel and $\Psi_i = K \Phi_i$. We thus consider 
\[
f = \sum_{j=1}^J w_j \Phi_j, ~ Kf = \sum_{j=1}^J w_j \Psi_j
\]

Denote by $(e_r)_r$ be the SVD basis associated with $K$ and $\sigma_r$ its eigenvalues ordered in the decreasing order. Denote for all $j,r$ 
\[ 
\Psi_{j,r} = \langle \Psi_j, e_r \rangle
\]
we deduce 
\[
\langle \Phi_j,\Phi_k\rangle = \sum_{r=1}^\infty \Psi_{j,r} \Psi_{k,r} \sigma^2_r 
\]
We now compute the modulus of continuity for this model. We have for every $r_n \in \N^* $ 
\begin{align*} 
\deux{Kf}^2 &= \sum_{j,k = 1}^J \left(  w_j w_k \sum_{r=1}^\infty \sigma_r^2 \Psi_{j,r}\Psi_{k,r} \right) \\ 
&= \sum_{j,k = 1}^J w_j w_k \left( \sum_{r = 1}^\infty (\sigma_r^2- \sigma_{r_n}^2) \Psi_{j,r}\Psi_{k,r} \right) + \sigma_{r_n}^2 \un{f}^2 \\ 
&= \sum_{r=1}^{\infty} (\sigma_r^2 - \sigma_{r_n}^2)  \left( \sum_{j=1}^J w_j\Psi_{j,r} \right)^2 + \sigma_{r_n}^2 \un{f}^2 \\ 
& \geq -\sigma_{r_n}^2 \sum_{r = r_n +1}^\infty \left(\sum_{j=1}^J w_j \Psi_{j,r}  \right)^2 + \sigma_{r_n}^2 \un{f}^2  
\end{align*}
We denote by $f_{r_n}$ the projection of $f$ onto the linear span of $\{e_1, \dots , e_{r_n} \}$. We thus have 
\begin{equation}
\deux{Kf}^2 \geq \sigma_{r_n}\left( \un{f}^2 - \un{f - f_{r_n}}^2  \right) = \sigma_{r_n}^2 \un{f_{r_n}}^2
\label{eq:modulus_mix_gen}
\end{equation}

Note that equation \eqref{eq:modulus_mix_gen} holds for any operator $K$ and any kernel $\Phi$. \\ 

We consider the circular convolution operator on $[0,2\pi]$ with convolution kernel $\lambda$, i.e. for all $f \in L_2([0,2\pi])$ 
$$
Kf(t) = \lambda \star f(t) = \int_0^{2\pi} \lambda(t-x)f(x) dx
$$
We choose a family of kernels $\Phi_j$ such that 
$$
K\Phi_j(x) = \Psi_j(x) = \frac{1}{\sqrt{2\pi v^2}} e^{-\frac{1}{2v^2}\left(x - 2\pi\frac{j}{J}\right)^2 }
$$
and put a prior $\Pi$ on $f$ such that the prior induce on $Kf$ satisfies the conditions of Theorem 2.2 of \citet{dejongvzanten12}. 

{\color{red} Is this interesting? Can we find an example for $\Phi$ and $\lambda$ ? Can we define the prior of $f$ through its Fourier coef? In this case we easily get 
$\Phi_j = \sum_k \Psi_{j,k}\sigma_k^{-1}$ }

Thus given that for the circular deconvolution, the SVD basis is known to be the Fourier basis, we can easily compute 
\[
	\Psi_{j,r} = e^{2\pi \frac{rj}{J}} e^{-\frac{r^2v^2}{2}}
\]
We thus have 
\[
	||f||^2 = \sum_{r=0}^\infty \left|\sum_{j=1}^J w_j e^{2i\pi{jr\over J}}  \right|^2 e^{-r^2v^2}
\]
As before we define $S_n = \left\{ ||f_{r_n}||^2 \geq c ||f||^2 \right\}$. We now prove that $\Pi(S_n^c) \leq C_2 e^{-C_3 n \epsilon_n^2}$. Denoting $c' = c/(1-c)$ we have

\begin{align*} 
	\Pi(S_n^c) &= \Pi\left( \sum_{r=0}^{r_n} e^{-r^2v^2} \left|\sum_{j=1}^J w_j e^{2i\pi{jr\over J}}  \right|^2 \leq c' \sum_{r=r_n +1}^{\infty} e^{-r^2v^2} \left|\sum_{j=1}^J w_j e^{2i\pi{jr\over J}}  \right|^2   \right) \\
\end{align*}

We have 
\begin{align*}
	||f_{r_n}||^2 &=	\sum_{r=0}^{r_n} e^{-r^2v^2} \left|\sum_{j=1}^J w_j e^{2i\pi{jr\over J}}  \right|^2 \\ 
          & \geq \sum_{r=1}^{r_n} e^{-r^2v^2} \left|\sum_{j=1}^J w_j e^{2i\pi{jr\over J}}  \right|^2 \\ 
	  & \geq \sum_{k=0}^{\floor{r_n/J}-1} \sum_{r = kJ +1}^{(k+1)J} e^{-r^2v^2} \left|\sum_{j=1}^J w_j e^{2i\pi{jr\over J}}  \right|^2 \\
	  & = \sum_{r=1}^{J}\left|\sum_{j=1}^J w_j e^{2i\pi{jr\over J}}  \right|^2 \sum_{k=1}^{\floor{r_n/J} - 1 } e^{-(r + kJ)^2v^2} \\
	  & \geq \sum_{r=1}^{J}\left|\sum_{j=1}^J w_j e^{2i\pi{jr\over J}}  \right|^2 {e^{-r^2v^2 - (\floor{r_n/J})^2v^2 }\over 1 - e^{-2rJv^2}} (1 - e^{-2Jv^2r\floor{r_n/J}}) \\ 
	  & \geq (1-e^{-2v^2(r_n-1)})\sum_{r=1}^{J}\left|\sum_{j=1}^J w_j e^{2i\pi{jr\over J}}  \right|^2 {e^{-r^2v^2 - (\floor{r_n/J})^2v^2 }\over 1 - e^{-2rJv^2}}  
\end{align*}
and similarly 
\begin{align*}
	||f_{r_n}^\perp||^2 &\leq \sum_{r = 1}^{J} \left|\sum_{j=1}^J w_j e^{2i\pi{jr\over J}}  \right|^2 \sum_{k = \floor{r_n/J}}^\infty e^{-(r + kJ)^2v^2} \\ 
	& \leq \sum_{r=1}^{J}\left|\sum_{j=1}^J w_j e^{2i\pi{jr\over J}}  \right|^2 {e^{-r^2v^2 - (\floor{r_n/J})^2v^2 }\over 1 - e^{-2rJv^2}} (e^{-2Jv^2r\floor{r_n/J}}) \\
	& \leq e^{-2v^2(r_n-1)}\sum_{r=1}^{J}\left|\sum_{j=1}^J w_j e^{2i\pi{jr\over J}}  \right|^2 {e^{-r^2v^2 - (\floor{r_n/J})^2v^2 }\over 1 - e^{-2rJv^2}}  
\end{align*}
we deduce 
\begin{align*}
	\Pi(S_n^c) &\leq \Pi\left( (1+c')e^{-2v^2(r_n - 1)} \geq 1 \right) \\ 
	& = \Pi\left( v^2 \leq C_4/(r_n-1) \right) \\ 
	& \lesssim e^{-C_5r_n \log(r_n)} 
\end{align*}
taking $r_n \asymp n^{1/(2\alpha + 2 \beta +1)}$ we get the desired result. 


==> Parts/old/some_examples_old.tex <==
%!TEX root = ../Inv_notes2.tex

In this section we first present an example of the sequence 
of sets $\mathcal{S}_n$, and later present how the modulus of 
continuity for this sequence can be computed in two standard 
inverse problem settings. We now suppose that $\mathcal{F}$ and 
$K\mathcal{F}$ are separable Hilbert spaces, 
denoted $(\H_1, \|\cdot\|_{\H_1})$ and $(\H_2,\|\cdot\|_{\H_2})$ 
respectively.

As already noted, the operator $K$ restricted to certain subsets of 
the domain $\H_1$ might have a finite modulus of continuity 
defined in (\ref{eq:def:modulus}). Clearly, one wants to construct 
a sequence of sets $\mathcal{S}_n$ that in a certain sense approaches 
the full domain $\H_1$. This is understood in terms of the 
remaining prior mass condition in Theorem~\ref{thm:main}. Moreover, since 
we do not require $f_0$ to be in $\mathcal{S}_n$, we need to be able to 
control the distance between $f_0$ and $\mathcal{S}_n$.  

A natural guess is to consider finite-dimensional projections of $\H_1$. 
In this section we go beyond this concept. To get some intuition, 
consider the Fourier basis of $\H_1$. The ill-posedness can be 
then viewed as too big an amplification of the high frequencies 
through the inverse of the operator $K$. Therefore, one wants 
to control the higher frequencies in the signal, and thus in 
the parameter $f$. 

Since $\H_1$ is a separable Hilbert space, there exist an 
orthonormal basis $(e_i)$ and each element $f \in \H_1$ 
can be viewed as an element of $\ell_2$ and
%
\[
%
    \un{f} = \sum_{i=1}^\infty f_i^2.
%
\]
%
For a given sequence $k_n \to \infty$ and a constant $c \geq 0$ we define
%
\begin{equation}
\label{eq:Sn}
%
    \mathcal{S}_n := 
       \Bigl\{f\in\ell_2: \sum_{i>k_n} f_i^2 \leq c\sum_{i \leq k_n}f_i^2\Bigr\}.
%
\end{equation}
%
We note that the finite-dimensional projections are also covered by this 
definition for $c = 0$. 

%\subsection{Singular value decomposition}
%\label{sec:SVD}
If the operator $K$ is compact, then the spectral decomposition of the 
self-adjoint operator $K^TK:\H_1 \to \H_1$ provides 
a convenient orthonormal basis. In the compact case the operator 
$K^TK$ possesses countably many positive eigenvalues $\kappa_i^2$ 
and there is a corresponding orthonormal basis $(e_i)$ of $\H_1$ 
of eigenfunctions, and the sequence $(\tilde e_i)$ defined by 
$Ke_i = \kappa_i\tilde e_i$ forms an orthonormal conjugate basis of the 
range of $K$ in $\H_2$. Therefore, both $f$ and $Kf$ can be associated 
with sequences in $\ell_2$. Since the problem is ill-posed when $\kappa_i \to 0$, 
we can assume without loss of generality that the sequence $\kappa_i$ is decreasing.

Let $k_n$ and $c$ in the definition of $\mathcal{S}_n$ be fixed. Then for any 
$g \in \mathcal{S}_n$
%
\begin{align*}
%
    \un{g}^2 &= \sum_{i=1}^\infty g_i^2 = \sum_{i \leq k_n}g_i^2  + \sum_{i > k_n}g_i^2 \\
       &\leq (1+c) \sum_{i \leq k_n}g_i^2  = (1+c) \sum_{i \leq k_n}\kappa_i^{-2}\kappa_i^2 g_i^2\\
       &\leq (1+c) \kappa_{k_n}^{-2}  \sum_{i \leq k_n}\kappa_i^2 g_i^2 \leq (1+c) \kappa_{k_n}^{-2}\deux{Kg}^2.
%
\end{align*}

Let $f_{n}$ be the projection of $f_0$ on the first $k_n$ coordinates, i.e., 
$f_{n,i} = f_{0,i}$ for $i \leq k_n$ and $0$ otherwise. Moreover, we assume 
that $f_0$ belongs to some smoothness class described by a decreasing sequence 
$(s_i)$:
%
\[
%
	\|f_0\|^2_s = \sum_{i=1}^\infty s_i^{-2}f_{0,i}^2 < \infty.
%
\]
%
The usual Sobolev space of regularity $\beta$ is defined in that way with 
$s_i = i^{-\beta}$. Therefore, we have
%
\[
%
	\|f_n-f_0\|_{\H_1} \leq s_{k_n}\|f_0\|_s, \qquad 
	\|Kf_n-Kf_0\|_{\H_2} \leq s_{k_n}\kappa_{k_n}\|f_0\|_s.
%
\]
%
Using the triangle inequality twice and keeping in mind that $f-f_n \in \mathcal{S}_n$ 
we obtain
%
\begin{align*}
%
	\|f-f_0\|_{\H_1} &\leq \|f-f_n\|_{\H_1} + \|f_n-f_0\|_{\H_1} \\
		& \leq \sqrt{1+c}\kappa_{k_n}^{-1}\|Kf-Kf_n\|_{\H_2} + s_{k_n}\|f_0\|_s\\
		& \leq \sqrt{1+c}\kappa_{k_n}^{-1}\bigl(\|Kf-Kf_0\|_{\H_2} + \kappa_{k_n}s_{k_n}\|f_0\|_s\bigr) 
			+ s_{k_n}\|f_0\|_s\\
		& = \sqrt{1+c}\kappa_{k_n}^{-1}\delta + \|f_0\|_s\bigl(1+\sqrt{1+c}\bigr)s_{k_n}.
%
\end{align*}
%
We then find an upper bound for the modulus of continuity, 
%
\begin{equation}
\label{eq:mod}
%
    \omega(\mathcal{S}_n,f_0, \|\cdot\|_{\H_1}, \|\cdot\|_{\H_2},\delta) \lesssim \kappa_{k_n}^{-1}\delta + s_{k_n}.
%
\end{equation}

\begin{remark}
If $c>0$, then $f_0 \in \mathcal{S}_n$ for $n$ large enough (depending on $f_0$). 
\end{remark}

\begin{remark}
These results generalize the ones presented in \cite{ray2013bayesian} for band limited wavelet prior. In this case, we do not ask the basis functions to have finite decomposition in the SVD but rather that their coefficients in the SVD decrease sufficiently fast. 
\end{remark}

% \subsection{Orthonormal basis of $L^2(\lambda)$}

% \bartek{Still to be rewritten. My previous comment (I don't know what I meant anymore): 
% I am not so sure whether this really makes a difference. 
% The $p-$times integration operator at the end of this subsection is no different 
% from SVD. Maybe another example?}

% For simplicity we will consider the case where $H = H_1 = H_2$. Let $e_i$ be an orthonormal basis of $H$, and consider $S = S(k) = \{ f = \sum_{i=1}^\infty f_i e_i , f_{k+p} = 0 \forall k >0 \}$. We thus have for all $f \in S(k)$
% $
% ||f||^2 = \int f(x)^2 d\lambda(x) = \sum_{i=1}^k f_i
% $
% and we have
% $
% ||Kf||^2 = \int Kf(x)^2 d \lambda(x) = \sum_{i,j} f_i f_j \int Ke_i(x)Ke_j(x) d\lambda(x)
% $
% Denoting $\f = (f_1, \dots , f_{k})$ and $\Sigma = \left(\int Ke_i(x)Ke_j(x) d\lambda(x) \right)$ we have
% $
% ||Kf||^2 = \f \Sigma \f'
% $
% Note that $\Sigma$ is a real symmetric matrix and can thus be diagonalized in an orthonormal basis (may be true with hermitian matrices/operator I will check on the Cavalier's book). Denote $\sigma_i$ its eigenvalues (in decreasing order). Thus
% \begin{equation}
% 	||Kf||^2 = \f \Sigma \f = \f P DP^{-1} \f' \geq \sigma_k^2 \f \f' = \sigma_k^2 ||f||^2
% \end{equation}
% Thus the modulus of continuity $\omega(S(k),||\cdot||, ||\cdot||, \epsilon) = \epsilon/\sigma_k$

% \paragraph{Application to the $p-$time integration operator and the Fourier basis}
% Consider the Fourier basis for $j \in \mathbb{Z}$, $e_j(x) = e^{ijx}$ and let $K$ be the $p-$times integration operator i.e. $Kf$ is such that $Kf^{(p)} = f$. Note that
% $
% Ke_j(x) = j^{-p}e^{ijx}
% $
% Thus $\Sigma$ is diagonal and $\sigma_k = k^{-p}$.



==> Parts/proofs_WN.tex <==
%!TEX root = ../inverse_general_BJ_rev.tex

\subsection{Additional proofs the mildly ill-posed case}
\label{sec:app:WN:mildly}


\begin{proof}[Proof of Lemma \ref{lem:mildlyKL}]
This proof is adapted from \citep{Belitser}. 
Recall that in the white noise model the $\ell_2$ balls and Kullback--Leibler
neighborhoods are equivalent. By independence, for any $N$, 
%
\begin{equation}
\label{eq:twoterms}
\begin{split}
%
    \Pi\Bigl(&\sum_{i=1}^\infty(\kappa_if_i-\kappa_if_{0,i})^2\leq \epsilon^2\Bigr)\\
        &\geq \Pi\Bigl(\sum_{i=1}^N(\kappa_if_i-\kappa_if_{0,i})^2\leq \epsilon^2/2\Bigr)
            \Pi\Bigl(\sum_{i=N+1}^\infty(\kappa_if_i-\kappa_if_{0,i})^2\leq \epsilon^2/2\Bigr).   
%
\end{split}
\end{equation}
%
Also
%
\begin{equation}
\label{eq:tailhelp}
%
    \sum_{i=N+1}^\infty(\kappa_if_i-\kappa_if_{0,i})^2 \leq 2\sum_{i=N+1}^\infty\kappa_i^2f_i^2
        + 2\sum_{i=N+1}^\infty\kappa_i^2f_{0,i}^2.
%
\end{equation}
%
The second sum in the display above is less than or equal to
%
\[
%
    2N^{-2\beta-2p}\sum_{i=N+1}^\infty i^{2\beta}f_{0,i}^2 
        \leq 2N^{-2\beta-2p}\|f_0\|_\beta^2 < \frac{\epsilon^2}{4},
%
\]
%
whenever $N > N_1 = (8\|f_0\|_\beta^2)^{1/(2\beta+2p)}\epsilon^{-1/(\beta+p)}$.

By Chebyshev's inequality, the first sum on the right-hand side of 
(\ref{eq:tailhelp}) is less than $\epsilon^2/4$ with probability at least
%
\[
%
    1-\frac{8}{\epsilon^2}\sum_{i=N+1}^\infty \E_{\Pi}(\kappa_i^2f_i^2) 
     = 1- \frac{8}{\epsilon^2}\sum_{i=N+1}^\infty i^{-1-2\alpha-2p} 
     \geq 1 - \frac{4}{(\alpha+p)N^{2(\alpha+p)}\epsilon^2}> 1/2
%
\]
%
if $N > N_2 = (8/(\alpha+p))^{1/(2\alpha+2p)}\epsilon^{-1/(\alpha+p)}$.

To bound the first term in (\ref{eq:twoterms}) we apply Lemma~6.2 in \cite{Belitser} 
with $\xi_i = \kappa_if_{0,i}$ and $\delta^2=\epsilon^2/2$. Note that
%
\begin{align*}
%
	\sum_{i=1}^Ni^{1+2\alpha+2p}\xi_i^2 &= \sum_{i=1}^Ni^{1+2\alpha+2p}\cdot i^{-2p}f_{0,i}^2 \\
	  &= \sum_{i=1}^Ni^{1+2\alpha-2\beta}f_{0,i}^2i^{2\beta} \leq N^{(1+2\alpha-2\beta)\wedge 0}\|f_0\|^2_\beta.
%
\end{align*}
%
Therefore,
%
\begin{align*}
%
    \Pi\Bigl(\sum_{i=1}^N(\kappa_if_i-&\kappa_if_{0,i})^2 \leq \epsilon^2/2\Bigr)\\
      &\geq \exp\Bigl(-\Bigl(1+2\alpha+2p+\frac{\log 2}{2}\Bigr)N\Bigr)
          \exp\Bigl(-N^{(1+2\alpha-2\beta)\wedge 0}\|f_0\|_\beta^2\Bigr)\\
      &\qquad \times{}
          \Pr\Bigl(\sum_{i=1}^N V_i^2 \leq 2\delta^2N^{1+2\alpha+2p}\Bigr).
%
\end{align*}
%
The last term, by the central limit theorem, is at least $1/4$ if $2\delta^2N^{1+2\alpha+2p}>N$ 
and $N$ is large, that is, $N > N_3 = \epsilon^{-1/(\alpha+p)}$ and $N > N_4$, where $N_4$ 
does not depend on $f_0$. Choosing $N = \max\{N_1, N_2, N_3, N_4\}$ we obtain
%
\begin{align*}
%
    \Pi(f:\|Kf-&Kf_0\|\leq \epsilon)\\
      &\geq \frac{1}{8}\exp\Bigl(-\Bigl(1+2\alpha+2p+\frac{\log 2}{2}\Bigr)N\Bigr)
          \exp\Bigl(-N^{(1+2\alpha-2\beta)\wedge 0}\|f_0\|_\beta^2\Bigr).
%
\end{align*}

Consider $\alpha \geq \beta$. Then $\exp(-N) \geq \exp(- N^{(1+2\alpha-2\beta)})$ so 
%
\[
%
    \Pi(f:\|Kf-Kf_0\|\leq \epsilon) \geq \frac{1}{8}
          \exp\Bigl(-C_3N^{(1+2\alpha-2\beta)}\Bigr),
%
\]
%
for some constant $C_3$ that depends only on $\alpha, \beta, p$ and $\|f_0\|_\beta^2$. Moreover, 
since $\epsilon < 1$ and $\alpha \geq \beta$, $N$ is dominated by $\epsilon^{-1/(\beta+p)}$ and 
we can write
%
\[
%
    \Pi(f:\|Kf-Kf_0\|\leq \epsilon) \geq \frac{1}{8}
          \exp\Bigl(-C_4\epsilon^{-\frac{1+2\alpha-2\beta}{\beta+p}}\Bigr), 
%
\]
%
where $C_4$ depends on $f_0$ again through $\|f_0\|_\beta^2$ only. 

Now consider $\alpha < \beta$. Similar arguments lead to 
%
\[
%
    \Pi(f:\|Kf-Kf_0\|\leq \epsilon) \geq \frac{1}{8}
          \exp\Bigl(-C_5\epsilon^{-\frac{1}{\alpha+p}}\Bigr), 
%
\]
%
for some constant $C_5$ that depends only on $\alpha, \beta, p$ and $\|f_0\|_\beta^2$.
\end{proof}





\begin{proof}[Proof of Lemma \ref{lem:mildlypriormass}]
For $W_1, W_2, \ldots$ independent standard normal random variables
%
\[
%
    \Pi(\mathcal{S}_n^c) = \Pr\Bigl(\sum_{i>k_n} \lambda_iW_i^2
            > c\rho_n^2\Bigr).
%
\]
%
For some $t > 0$
%
\begin{align*}
%
    \Pr\Bigl(&\sum_{i>k_n} \lambda_iW_i^2
            > c\rho_n^2\Bigr)\\
        &= \Pr\Bigl(\exp\Bigl(t\sum_{i>k_n} \lambda_iW_i^2\Bigr)
            > \exp(tc\rho_n^2)\Bigr)
        \leq \exp(-tc\rho_n^2)
            \E \exp\Bigl(t\sum_{i>k_n} \lambda_iW_i^2\Bigr)\\
%        &= \exp(-tc\rho_n^2)
%            \E\prod_{i>k_n} \exp(t\lambda_iW_i^2)\\
        &= \exp(-tc\rho_n^2)
            \prod_{i>k_n} \E\exp(t\lambda_iW_i^2)
        = \exp(-tc\rho_n^2)
            \prod_{i>k_n} (1-2t\lambda_i)^{-1/2}.
%
\end{align*}
%
We first applied Markov's inequality, and later used properties of
the moment generating function. Here we additionally assume
that $2t\lambda_i < 1$ for $i > k_n$.

We take the logarithm of the right-hand side of the
previous display. Since $\log(1-y)\geq -y/(1-y)$, we have
%
%
\begin{align*}
%
    -tc\rho_n^2 + &\sum_{i>k_n}\log (1-2t\lambda_i)^{-1/2}\\
        &=  -tc\rho_n^2
            - \frac{1}{2} \sum_{i>k_n}\log (1-2t\lambda_i)
        \leq -tc\rho_n^2
            + \frac{1}{2} \sum_{i>k_n}\frac{2t\lambda_i}{1-2t\lambda_i}.
%
\end{align*}
%
We continue with the latter term, noticing that $1-2t\lambda_i > 1-2tk_n^{-1-2\alpha}$ 
for $i > k_n$
%
\[
%
	\frac{1}{2} \sum_{i>k_n}\frac{2t\lambda_i}{1-2t\lambda_i} \leq 
	   \frac{t}{1-2tk_n^{-1-2\alpha}} \sum_{i>k_n}i^{-1-2\alpha}.
%
\]
%
Since $x^{-1-2\alpha}$ is decreasing, 
we have that
%
\[
%	
	\sum_{i>k_n}i^{-1-2\alpha} \leq \int_{k_n}^\infty x^{-1-2\alpha}\, dx + k_n^{-1-2\alpha} 
	  = \frac{k_n^{-2\alpha}}{2\alpha} + k_n^{-1-2\alpha} \leq k_n^{-2\alpha} \frac{1+2\alpha}{2\alpha}, 
%
\]
%
noting that $k_n > 1$ for $n$ large enough. Finally
%
\[
%
	    -tc\rho_n^2
            + \sum_{i>k_n}\log (1-2t\lambda_i)^{-1/2} 
            \leq -tc\rho_n^2
            + \frac{1+2\alpha}{2\alpha}
                \frac{t}{1-2tk_n^{-1-2\alpha}} k_n^{-2\alpha}.
%
\]
%
Thus for $t = k_n^{1+2\alpha}/4$
%
\[
%
    \Pi(\mathcal{S}_n^c)\leq \exp\Bigl(-\frac{c}{4}\rho_n^2k_n^{1+2\alpha} + \frac{1+2\alpha}{4\alpha}k_n\Bigr) 
	\leq \exp\Bigl(-\frac{c}{8}\rho_n^2k_n^{1+2\alpha}\Bigr), 
%
\]
%
since $k_n^{2\alpha} \geq 2(1+2\alpha)/(\alpha c\rho_n^2)$.
\end{proof}


\subsection{Additional proofs the severely and extremely ill-posed case}
\label{sec:app:WN:extremely}


\begin{proof}[Proof of Lemma \ref{lem:inequalities}]
Note that $t_{i,n} \leq n^{-1}$ and $s_{i,n} \leq n^{-1}$. 
Therefore, the last two sums in (\ref{eq:asymptotics}) are bounded from 
above by $n^{-1}k_n = n^{-1}(\log n)^{1/p}$.

As for the first term in the first sum in (\ref{eq:asymptotics}) we have
%
\[
\begin{split}
%
	\sum_{i\leq k_n} \frac{\kappa_i^2f_{0,i}^2}{(1+n\lambda_i\kappa_i^2)^2} &\leq 
	n^{-2} \sum_{i\leq k_n} \lambda_i^{-2}\kappa_i^{-2}i^{-2\beta}i^{2\beta}f_{0,i}^2\\
	&= n^{-2} \sum_{i\leq k_n} i^{2(\alpha-\beta)}\exp(2(\xi+\gamma)i^p)i^{2\beta}f_{0,i}^2,
%
\end{split}
\]
%
and for $k_n$ large enough all terms $i^{2(\alpha-\beta)}\exp(2(\xi+\gamma)i^p)$ are dominated 
by $k_n^{2(\alpha-\beta)}\exp(2(\xi+\gamma)k_n^p)$, so
%
\begin{equation}
\label{eq:firstsum}
%
	\sum_{i\leq k_n} \frac{\kappa_i^2f_{0,i}^2}{(1+n\lambda_i\kappa_i^2)^2} \leq
	 n^{-2}k_n^{2(\alpha-\beta)}\exp(2(\xi+\gamma)k_n^p)\|f_0\|^2_\beta.
%
\end{equation}

As for the second term in the first sum in (\ref{eq:asymptotics}) we note that
%
\[
%
	\sum_{i > k_n} \kappa_i^2 f_{0,i}^2 = \sum_{i > k_n} \exp(-2\gamma i^p)i^{-2\beta}i^{2\beta} f_{0,i}^2,
%
\]
%
and since $\exp(-2\gamma i^p)i^{-2\beta}$ is monotone decreasing
%
\begin{equation}
\label{eq:secondsum}
%
	\sum_{i > k_n} \kappa_i^2 f_{0,i}^2 
	  \leq \exp(-2\gamma k_n^p)k_n^{-2\beta}\|f_0\|^2_\beta.
%
\end{equation}

Recall that $\exp(k_n^p) = (nk_n^{-\alpha})^{1/(\xi+2\gamma)}$  
and therefore we can rewrite the bounds in (\ref{eq:firstsum}) and (\ref{eq:secondsum}) 
as
%
\[
%
	n^{-2}k_n^{2(\alpha-\beta)}\bigl(nk_n^{-\alpha}\bigr)^{\frac{2(\xi+\gamma)}{\xi+2\gamma}} =  
	n^{-\frac{2\gamma}{\xi+2\gamma}} k_n^{-2\beta + \frac{2\gamma\alpha}{\xi+2\gamma}},
%
\]
%
and
%
\[
%
	k_n^{-2\beta}\bigl(nk_n^{-\alpha}\bigr)^{-\frac{2\gamma}{\xi+2\gamma}} = 
	n^{-\frac{2\gamma}{\xi+2\gamma}} k_n^{-2\beta + \frac{2\gamma\alpha}{\xi+2\gamma}}.
%
\]
%
Finally, since $k_n$ in this case can be taken of the order $(\log n)^{1/p}$, we obtain the 
desired upper bound.
\end{proof}




==> Parts/proofs_regression.tex <==
%!TEX root = ../inverse_general_BJ_rev.tex

\subsection{Additional proofs for numerical integration}
\label{sec:app:regression:numerical:integration}


\begin{proof}[Proof of Lemma \ref{lem:adapt:cvrate:splines}]
We prove Lemma \ref{lem:adapt:cvrate:splines} using Theorem 4 in \citep{GhosalVdv07}. 
Let $\beta \leq q$ and $f_0$ be in $\mathcal{H}(\beta,L)$ and set 
$\epsilon_n = C n^{-(\beta+1)/(2\beta +3)} (\log n)^r$ with $r = (1\vee t)\beta/(2\beta +1)$. 
Set $J_n := J_0 n \epsilon_n^{2} \log(n)^{-t}$ for a fixed constant $J_0>0$ and 
consider the sets $\mathcal{S}_n$ defined by 
%
\[
%
	\mathcal{S}_n := \bigl\{ J \leq J_n, a \in \R^J\bigr\}
%
\]
%
We first control the local entropy function 
$N(\epsilon, \{ J,a \in \mathcal{S}_n : \|Kf - Kf_0\|_n \leq \epsilon_n \} ,\|\cdot\|_n)$. 
By using the same reasoning as in the proof of Theorem 12 in \citep{GhosalVdv07}, for all $J \in S_n$ we get
%
\[
%
	\log(N(\epsilon, \{ J,a \in \mathcal{S}_n : \|Kf - Kf_0\|_n \leq \epsilon_n \} , \|\cdot\|_n) )\leq n \epsilon_n^2.
%
\]
%
The prior mass of the set $\mathcal{S}_n$ is easily controlled using condition 
(\ref{eq:regression:volterra:conditionJ}):
% 
\[
%
	\Pi(\mathcal{S}_n^c) = \Pi_J(J > J_n) \leq \exp(-c_u J_n (\log J_n)^t). 
%
\]
%
We now need to control the prior mass of Kullback--Leiber neighborhoods of $Kf_0$. 
Note that this condition will also be useful to apply Lemma \ref{lem:main} and 
thus derive the posterior contraction rate for the direct problem.
Let $B_n(Kf_0, \epsilon)$ be defined as in (\ref{eq:main:de:KLneighbour}). 

Using the results of Section 7.3 in \citep{GhosalVdv07}, setting $\tilde{J}_n = J_n (\log n)^{-r/\beta}$ 
we deduce that for some constant $c$ depending only on $\sigma$ 
%
\[
%
	B_n(Kf_0,\epsilon_n) \supset \{ \tilde{J}_n \leq J \leq 2 \tilde{J}_n, \|Kf - Kf_0\|_n^2 \leq c\epsilon_n^2 \}.
%
\]
%
Standard approximation results on splines give that for all $J$ there exists a 
sequence $a_0= (a_{0,1}, \dots , a_{0,J})$ such that 
%
\[
%
	\Bigl\|Kf_0 - \sum_{j=1}^J a_{0,j} B_{j,q} \Bigr\|_n \leq J^{-\beta -1} \|Kf_0\|_\beta \leq J^{-\beta -1} L.
%
\]
% 
Given condition {\bf D1} on the design, we thus have that for a constant $c'>0$ 
depending only  on $\sigma$ and $L$
%
\[
%
	B_n(Kf_0,\epsilon_n) \supset 
		\bigl\{ \tilde{J}_n \leq J \leq 2 \tilde{J}_n, \|a-a_0\|_{\tilde{J}_n} \leq c' \tilde{J}_n^{1/2} \epsilon_n \bigr\}.
%
\]
%
Therefore, we obtain a lower bound on the prior mass of a Kullback--Leibler 
neighbourhood of $Kf_0$:
%
\[
\begin{split}
%
	\Pi(B_n(Kf_0,\epsilon_n)) &\geq 
			\Pi\bigl( \tilde{J}_n \leq J \leq 2\tilde{J}_n, \|a - a_0 \|_n \leq  c'\tilde{J}_n^{1/2} \epsilon_n \bigr) \\
		&\geq \exp\bigl(- \tilde{J}_n ( c_d(\log \tilde{J}_n)^t + c_2 \log(\tilde{J}_n^{-1/2}\epsilon_n^{-1}))\bigr).
%
\end{split}
\]
%
We thus have for $C_2>0$,
%
\begin{equation}
%
	\frac{\Pi(\mathcal{S}_n^c)}{\Pi(B_n(Kf_0,\epsilon_n))} \leq \exp(-C_2 J_n (\log J_n)^t), 
%
\end{equation}
%
which together with Theorem 4 in \citep{GhosalVdv07} ends the proof. 
\end{proof}


\subsection{Additional proofs for deconvolution}
\label{sec:app:regression:deconvolution}

\begin{proof}[Proof of Lemma \ref{lem:theotherlemma}]

We now adapt the results of \citep{dejongvzanten12} to our setting in order 
to control the posterior mass of the Kullback--Leibler neighbourhoods of $Kf_0$ 
and the posterior contraction rate for the direct problem. 
Following their notation we have that $K\Psi_v \in \mathcal{P}_\infty$, 
and thus the small ball probability $\Pi(\|f\|_\infty \leq \epsilon)$ 
can be controlled by their Lemma 3.3. We then extend their Lemma 3.5 to our setting. 
Note that with Lemma 9 of \citep{scricciolo2014adaptive}, 
Lemma 3.4 of \citep{dejongvzanten12} holds for the same $T_{\alpha,v}$ with $\alpha = \beta + p$. 
Choosing $h$ to be as in the proof of Lemma 3.5 of \citep{dejongvzanten12} and denoting 
$\omega_0 = f_0 \star \lambda$, we have 
%
\[
%
	h(x) = \sum_{j/J \in [-2c_x \log n, 2c_x \log n]} 
			T_{\alpha,v}(\omega_0) \frac{1}{J v} \Psi\Bigl( \frac{x-j/J}{v} \Bigr),
%
\]
%
and thus deduce 
%
\[
%
	\|h\|^2_{H^{J,v}} \leq 2c_x \|T_{\alpha,v}(\omega_0)\|^2  \log n.
%
\]
%
Using their decomposition (3.8), we control 
$|h(x) - \Psi_v \star T_{\alpha,v}(\omega_0)(x)|$ along the same lines 
as in their computations on page 3312. We have 
%
\[
\begin{split}
%
	&|h(x) - \Psi_v \star T_{\alpha,v}(\omega_0)(x)|\\
		&\qquad \leq \Bigl|h(x) - \int_{-2c_x \log n}^{2c_x \log n} T_{\alpha,v}(\omega_0)(y) \Psi_v(x-y) dy \Bigr|  \\ 
		&\qquad + \Bigl| \int_{-\infty}^{-2c_x \log n} T_{\alpha,v}(\omega_0)(y) \Psi_v(x-y) dy \Bigr|  
		   + \Bigl|\int_{2c_x \log n}^\infty T_{\alpha,v}(\omega_0)(y) \Psi_v(x-y) dy\Bigr|
%
%\label{eq:regression:deconv:proof:approx}
\end{split}
\]
%
The first term on the right hand side of the above display can be controlled as in the proof of Lemma 3.5 of \citep{dejongvzanten12}. 
For the last two terms, we have 
%
\[
\begin{split}
%
	\Bigl| \int_{-\infty}^{-2c_x \log n} &T_{\alpha,v}(\omega_0)(y) \Psi_v(x-y) dy \Bigr| 
		+  \Bigl|\int_{2c_x \log(n)}^\infty T_{\alpha,v}(\omega_0)(y) \Psi_v(x-y) dy\Bigr| \\ 
		&\lesssim \|T_{\alpha,v}(\omega_0)\|_\infty e^{-\frac{c_x^2 (\log n)^2}{2v^2} } v^{-1}.
%
\end{split}
\]
%
Following the same proof of Theorem 2.2 of \citep{dejongvzanten12}, we get
%
\[
%
	\E_0\Pi(\|Kf - Kf_0\| \geq C n^{-\frac{\beta + p}{1+2\beta + 2p}} (\log n)^{r} |Y^n) \to 0,  
%
\]
%
and similarly to their equation (2.5) we get, 
with $\epsilon_n =  n^{-(\beta + p)/(1+2\beta + 2p)} (\log n)^{r}$, 
where $r$ is some constant, 
%
\[
%
	\Pi(\|Kf-Kf_0\| \leq  \epsilon_n ) \geq e^{-n\epsilon_n^2}.
%
\]
%


\end{proof}
